Serverless data pipeline approaches for IoT data in fog and cloud computing

With the increasing number of Internet of Things (IoT) devices, massive amounts of raw data is being generated. The latency, cost, and other challenges in cloud-based IoT data processing have driven the adoption of Edge and Fog computing models, where some data processing tasks are moved closer to data sources. Properly dealing with the flow of such data requires building data pipelines, to control the complete life cycle of data streams from data acquisition at the data source, edge and fog processing, to Cloud side storage and analytics. Data analytics tasks need to be executed dynamically at different distances from the data sources and often on very heterogeneous hardware devices. This can be streamlined by the use of a Serverless (or FaaS) cloud computing model, where tasks are defined as virtual functions, which can be migrated from edge to cloud (and vice versa) and executed in an event-driven manner on data streams. In this work, we investigate the benefits of building Serverless data pipelines (SDP) for IoT data analytics and evaluate three different approaches for designing SDPs: 1) Off-the-shelf data flow tool (DFT) based, 2) Object storage service (OSS) based and 3) MQTT based. Further, we applied these strategies on three fog applications (Aeneas, PocketSphinx, and custom Video processing application) and evaluated the performance by comparing their processing time (computation time, network communication and disk access time), and resource utilization. Results show that DFT is unsuitable for compute-intensive applications such as video or image processing, whereas OSS is best suitable for this task. However, DFT is nicely fit for bandwidth-intensive applications due to the minimum use of network resources. On the other hand, MQTT-based SDP is observed with increase in CPU and Memory usage as the number of...<truncted to fit character limit in Arxiv>

==> DPIoT.tex <==
%     3.1. short background on new DP solutions (nifi, industrial solutions, etc)
%     3.2. challenges with current platform (serverless, fog and cloud, IoT etc)
%     Serverless DP
%     Introduce all the approaches with short description
\section{Background}\label{sec:background}

% In this section, we describe the background of modern data pipeline solutions with their challenges and benefits. We also provide preliminary analysis on current serverless data pipeline technologies and thier implications on IoT data processing. Finally, we outlined an existing data handling mechanisms that can be integrated with serverless framework.

%\subsection{State of art in data pipeline solutions}

%It allows the developers to model the flow of data from source to sink, while facilitating the hassle free design of pipelines for intermediate data operations. While, data movement from source to sink meaning that, either copied, transferred between storage repositories, reformatted for each system, and/or integrated with other data sources. A comprehensive data pipeline can help the system to work together. Moreover, data pipelines can process continuous, batch or stream processing applications. 


%A typical data pipeline consists of three elements, data source, sink and operators/components in the middle. A source is a data generator such as relation databases, events in web activities, SaaS applications, etc.,. The data can be collected from source via Message Queues such as  MQTT or Kafka or via REST API calls. A sink is a consumer of the processed data such as a data store,  Machine Learning models, data warehouses, BI tools or cloud hosted application such as visualization  and reporting tools. The components or  operators are set of processors capable to perform actions on the data. An application which helps to construct such kind of data pipelines is know as DP tool/engine.

%Moreover, data pipelines are used to process continuous, batch or stream processing applications. 







% ...markets and use of appropriate DP tool significantly varies according to the domain and use cases as described in Table \ref{DPTools}. On the other-line, DP tools are  significantly used in enterprises due to an ever-growing amounts data and increasing demands in data warehouse \& analytics for building a railroad pipelines to operate on data oriented business processes.In such cases, ETL(Extract, Load Transform) is more prevalent to ensure an integration between multiple databases and applications.

%They are significantly used in big-data analytics, data science and Machine Learning applications(CRM, social media and banking analytics, etc.) for raw data collection, cleaning, etc. and 

On the other hand, IoT is new driving force in  Industry 4.0 innovation. It's landscape is rapidly evolving with diverse applications including smart home, predictive maintenance, real-time telemetry and healthcare, etc. The developers and stakeholders of the ecosystem are finding a new way to drive their data to make faster decisions. On this context, Data pipelines are  more prevalent in handling the data in IoT environments. More precisely, Several cloud centric IoT data processing techniques solutions had been proposed  Djonov et.al\cite{djonov2020real} proposed cloud centric pipeline using AWS IoT for digital twin, Rashid et.al propsoed a secuirty model for IoT data procesinf at clouds, Samant ert.al \cite{8457831} designed a QoS model for execution of IoT DP in clouds

%More precisely, IoT data pipelines are constructed and executed in cloud environments\cite{}. such as in AWS IoTin data can be dirty or with different format or can have missing values while ingesting from different  sources. 
Data can be dirty when it’s ingested. Missing values or nonsensical values from sensors or device components are possible. Also, as is the case with any messaging architecture, the QoS of the message delivery mechanism can vary. Suppose IoT devices are communicating over HTTP via a WiFi connection directly to AWS or Azure. Intermittent drops in coverage or the internet connection may cause duplicate messages to be delivered. As mentioned in Gathering Data, if ingested messages are processed by Azure Functions or AWS Lambdas, the code can filter for dirty data or duplicate messages
%Workflows


%Different requirements may require orchestration of data flowing among different components with conditional logic. Custom calculations or complex algorithms may operate against data streams. Machine learning algorithms may require access to recently ingested IoT data in order to make predictions. Alternatively, microservices may pre-calculate values for reporting applications to improve performance. A more involved chain of components may execute to route, transform and operate on data. In AWS, Data Pipelines and Step Functions allow workflows to be created. Similarly in Azure, Data Factory and Logic Apps are applicable workflow tools.  Loosely coupling services with Azure Service Bus or AWS SNS/SQS ensures good architectural practices. 
% Example of pipeline
DP engines have a flexibility to extend the services to run on edge devices and perform data operation near to the source. This has more advantage in IoT systems for reducing latency and bandwidth consumption in complex applications. Apache Nifi has light weight version known as \textit{MiniFi} that can run on edge devices and manged centrally. that supports to perform pre-processing operations in edge devices. Stream-Set has lighter version called \textit{SDC Edge}. It's used read data from an edge device or to receive data from another pipeline and then act on that data to control an edge device.

In our proposed work, we have chosen Apache Nifi as DP engine as it's simple, flexible components(or processors) and widely used in commercial  big data platforms such as Hortanworks[]. Evermore, it has light weight version known as MiniFi[] that can run on edge devices that supports to perform pre-processing operations near to the data source to reduce latency and bandwidth, cost of execution. It also facilitates the automated deploy and management  of multiple MiniFi's running at different edge devices.
%\subsection{Challenges in current DP platforms}
%\subsection{Serverless data pipeline}
%\subsection{Proposed SDP approaches}
